KiDS+VIKING-450 and DES-Y1 combined: Mitigating baryon feedback uncertainty with COSEBIs

We present cosmological constraints from a joint cosmic shear analysis of the Kilo-Degree Survey (KV450) and the Dark Energy Survey (DES-Y1), conducted using Complete Orthogonal Sets of E/B-Integrals (COSEBIs). With COSEBIs we isolate any B-modes which have a non-cosmic shear origin and demonstrate the robustness of our cosmological E-mode analysis as no significant B-modes are detected. We highlight how COSEBIs are fairly insensitive to the amplitude of the non-linear matter power spectrum at high $k$-scales, mitigating the uncertain impact of baryon feedback in our analysis. COSEBIs, therefore, allow us to utilise additional small-scale information, improving the DES-Y1 joint constraints on $S_8=\sigma_8(\Omega_{\rm m}/0.3)^{0.5}$ and $\Omega_{\rm m}$ by $20\%$. Adopting a flat $\Lambda$CDM model we find $S_8=0.755^{+0.019}_{-0.021}$, which is in $3.2\sigma$ tension with the Planck Legacy analysis of the cosmic microwave background.

==> discussion.tex <==
\label{sec:discussion}


